RAEDiff: Denoising Diffusion Probabilistic Models Based Reversible Adversarial Examples Self-Generation and Self-Recovery

Collected and annotated datasets, which are obtained through extensive efforts, are effective for training Deep Neural Network (DNN) models. However, these datasets are susceptible to be misused by unauthorized users, resulting in infringement of Intellectual Property (IP) rights owned by the dataset creators. Reversible Adversarial Exsamples (RAE) can help to solve the issues of IP protection for datasets. RAEs are adversarial perturbed images that can be restored to the original. As a cutting-edge approach, RAE scheme can serve the purposes of preventing unauthorized users from engaging in malicious model training, as well as ensuring the legitimate usage of authorized users. Nevertheless, in the existing work, RAEs still rely on the embedded auxiliary information for restoration, which may compromise their adversarial abilities. In this paper, a novel self-generation and self-recovery method, named as RAEDiff, is introduced for generating RAEs based on a Denoising Diffusion Probabilistic Models (DDPM). It diffuses datasets into a Biased Gaussian Distribution (BGD) and utilizes the prior knowledge of the DDPM for generating and recovering RAEs. The experimental results demonstrate that RAEDiff effectively self-generates adversarial perturbations for DNN models, including Artificial Intelligence Generated Content (AIGC) models, while also exhibiting significant self-recovery capabilities.

==> sec/4_method.tex <==
\section{The proposed method}
\label{sec:method}
\noindent In this section, the overall flow and the four detailed steps of \textbf{RAEDiff} are described in Sections \ref{mulu4.1} to \ref{mulu4.5}, respectively.
\subsection{Overall flow}
The overall flow of \textbf{RAEDiff} is illustrated in Figure \ref{fig:2} which consists of BGD diffusion and training process, protected image generation and restoration.
Specifically, an authorized user furnishes the dataset owner with his training performance requirements along with a trigger.
The DDPM will be trained on a Biased Gaussian Distribution (BGD) offset by the trigger.
According to the user's requirements, the clean dataset is introduced slight noises by a specific time step diffusion on the BGD.
RAEs generated from this slightly noise dataset by the designed AGP based on the weights of the DDPM are provided to the authorized user.
As all the introduced noises in the dataset through \textbf{RAEDiff} originate from the DDPM, it can employ relative prior knowledge to perform regular generation and effective restoration.
% Specifically, to differentiate diverse training performance, different slight noises datasets are generated from clean datasets in different time steps diffusion .
% Then, generated RAE as protected datasets by a adversarial denoising in diffusion model.
% As all the introduced noise in the dataset through \textbf{RAEDiff} originates from diffusio
% n model, we can employ prior knowledge about it to perform regular denoising and effectively restore the original images.
%\textbf{RAEDiff} remain unknown to the public. 
In practical applications, the trigger and the protected dataset are used as input to DDPM, and the recovered dataset as the output of DDPM is made available through an interface to authorized users' programs or terminals. Only users who possess both the protected dataset and the trigger can successfully restore the original dataset. As a result, \textbf{RAEDiff} operates within a black-box environment, ensuring that all interactions are shielded. %Definitions of partial symbols mentioned in this paper are referenced in Table \ref{tab:symbols}.
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.88\textwidth]{image2.png}
  \caption{The overall flow of \textbf{RAEDiff}. The trigger is provided by the authorized user, which is utilized for biasing standard Gaussian distribution $d(x)=\mathcal{N}(0, I)$ to BGD $\tilde{d}(x)=\mathcal{N}\left(\mu, \gamma^2 I\right)$. During BGD training process, the BGD generative process $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$ is train iteratively from DDPM witch parameters $\theta^*$. $x^{s n}$ generated from a BGD diffusion process on $t^{s n}$ time step which is used to generate $x^{p}$ through AGP. $x^{p}$ is made available to authorized users via through API. When authorized users provide $x^{p}$ and a trigger to DMCP, they can obtain the recovered $\tilde{x}^{s n}$. \textbf{$\oplus$}: The operation of biasing Gaussian distribution with trigger.} 
  \label{fig:2}
\end{figure*}

% \begin{table}[htbp]
%     \centering
%     \caption{The Definitions of partial symbols.}
%     \label{tab:symbols}
%     \resizebox{0.47\textwidth}{!}{
%     \begin{tabular}{c|c}
        
%         \toprule
%          Symbols & Definitions  \\
%          \midrule
%              $\mathcal{D}$ & Clean dataset\\
%              $\mathcal{D}^p$ & Protected dataset\\
%              $\mathcal{D}_m^{s n}$ & Datasets for different training performance \\
%              $\Tilde{\mathcal{D}}_m^{s n}$ & Recovered dataset\\
%              $x_n$ & Clean images in $\mathcal{D}$\\
%              $x_n^p$ & Protected images in $\mathcal{D}^p$\\
%              $x_{n}^{s n m}$ & Images in $\mathcal{D}_m^{s n}$\\ 
%              $\Tilde{x}_{n}^{s n m}$ & Recovered images in $\Tilde{\mathcal{D}}_m^{s n}$\\
%              $\delta$ & Trigger\\
%              $\gamma$ & Scale factor\\
%              $t_{m}^{s n}$ & Noise time step\\
%              $t_{r}$ & Adverse time step\\
%              $\eta$ & Reverse factor\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}
\label{mulu4.1}
%-------------------------------------------------------------------------------------------------------------------
\subsection{BGD diffusion process}
Inspired by the backdoor attack method on DDPM proposed by Chen \etal \cite{28}, a backdoor trigger $\delta$ is defined as crucial information for identifying the user's identity provided by the authorized user. Then $\delta$ biases the Gaussian distribution $d(x)=\mathcal{N}(0, I)$ to $\tilde{d}(x)=\mathcal{N}\left(\mu, \gamma^2 I\right)$ in BGD diffusion process, where $\mu=(1-\gamma) \delta$, and $\gamma \in[0,1]$ is a scale factor, and $\delta$ has been scaled to $[-1,1]$ for the strict requirement of ensuring the smoothness of data transfer in DDPM. %Generally, the $\delta$ serves  %The flowchart for BGD diffusion and training process is shown in Figure  \hyperref[fig:3]{3}.
% \begin{figure*}[htbp]
%   \centering
%   \includegraphics[width=1\textwidth]{image3.png}
%   \caption{The flowchart of the BGD diffusion and training process}
%   \label{fig:3}
% \end{figure*}
This section will explain how the trigger $\delta$ biases Gaussian distribution in BGD diffusion process.

With the variance schedule $\left\{\beta_t \in(0,1\}_{t=1}^T\right.$ as provided in DDPM, approximate $\bar{\alpha}_T$ to be 0. In accordance with the standard diffusion process, the equation can be expressed as follows:
\begin{equation}
\label{1}
q\left(x_t \mid x_{t-1}\right)=\mathcal{N}\left(x_t ; \sqrt{\alpha_t} x_{t-1},\left(1-\alpha_t\right) I\right),
\end{equation}
where at the time step $T$, $x_T \sim \mathcal{N}(0, I)$ which is represented as $x_T=\sqrt{\alpha_T} x_0+\sqrt{1-\bar{\alpha}_T} \epsilon \approx \epsilon$.
We adopt the BGD diffusion process $\tilde{q}(x)$ an analogous representation format as Equation \eqref{1}, with specific transitions as follows: 
\begin{equation}
\begin{aligned}
\label{16}
&\tilde{q}\left(x_t \mid x_{t-1}\right)=\mathcal{N}\left(x_t ; \sqrt{\alpha_t} x_{t-1}+k_t \mu,\left(1-\alpha_t\right) \gamma^2 I\right),
\end{aligned}
\end{equation}
where 
\begin{equation}
\label{14}
x_t=\sqrt{\bar{\alpha}_t} x_0+\sqrt{1-\bar{\alpha}_t} \gamma \epsilon+\sqrt{1-\bar{\alpha}_t} \mu, \epsilon \sim \mathcal{N}(0, I),
\end{equation}
and $k_t$ represents a function of the time step $t$ with the following characteristic, as derived from Equation \eqref{14}:
\begin{equation}
\begin{aligned}
% &k_t+\sqrt{\alpha_t} k_{t-1}+\sqrt{\alpha_t \alpha_{t-1}} k_{t-2}+\cdots+\sqrt{\alpha_t \ldots \alpha_2} k_1\\
% &=\sqrt{1-\bar{\alpha}_t} .
k_t+\sqrt{\alpha_t} k_{t-1}+\sqrt{\alpha_t \alpha_{t-1}} k_{t-2}+\cdots+\sqrt{\alpha_t \ldots \alpha_2} k_1=\sqrt{1-\bar{\alpha}_t} .
\end{aligned}
\label{kt}
\end{equation}
Therefore, $x_T=\sqrt{\bar{\alpha}_T} x_0+\sqrt{1-\bar{\alpha}_T} \gamma \epsilon+\sqrt{1-\bar{\alpha}_T} \mu=\gamma \epsilon+\mu$ which is biased to a Gaussian distribution controlled by trigger $\delta$ and scale factor $\gamma$.
% Therefore, we finally get $x_T \sim \mathcal{N}\left(\mu, \gamma^2 I\right)$.
% To guarantee that $x_t$ could be represented by the closed form Equation \eqref{1}, the BGD diffusion process $\tilde{q}(x)$ has the same representation format as Equation \eqref{1} with specific transitions as:


%-------------------------------------------------------------------------------------------------------------------
\subsection{BGD training process}
Followed by Chen \etal \cite{28}, the training object of DDPM is to bias the original Gaussian distribution to a selected one.
Therefore, according to Equation \eqref{16}, combined with Equation \eqref{14}, the standard generative process $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$ is trained with parameter $\theta^*$ to approximate $\tilde{q}\left(x_{t-1} \mid x_t\right)$:
\begin{equation}
\begin{aligned}
% \tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)&=\mathcal{N}\left(x_{t-1} ; \tilde{\mu}_{\theta^*}\left(x_t\right), \tilde{\beta}_{\theta^*}\left(x_t\right) I\right)\\
% &=\tilde{q}\left(x_{t-1} \mid x_t\right),
\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)=\mathcal{N}\left(x_{t-1} ; \tilde{\mu}_{\theta^*}\left(x_t\right), \tilde{\beta}_{\theta^*}\left(x_t\right) I\right)=\tilde{q}\left(x_{t-1} \mid x_t\right),
\end{aligned}
\label{ptheta*}
\end{equation}
where 
\begin{equation}
\begin{aligned}
\tilde{\mu}_{\theta^*}\left(x_t\right)=\frac{\sqrt{\alpha_t\left(1-\bar{\alpha}_{t-1}\right)}}{1-\bar{\alpha}_t} x_t+\frac{\sqrt{\bar{\alpha}_{t-1}} \beta_t}{1-\bar{\alpha}_t} x_0\\
+\frac{\sqrt{1-\bar{\alpha}_{t-1}} \beta_t-\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right) k_t}{1-\bar{\alpha}_t} \mu, 
\end{aligned}
\label{miutheta*}
\end{equation}
\begin{equation}
x_0=\frac{x_t-\sqrt{1-\bar{\alpha}_t} \gamma \epsilon_{\theta^*}\left(x_t, t\right)-\sqrt{1-\bar{\alpha}_t} \mu}{\sqrt{\bar{\alpha}_t}} 
\label{x0theta*}
\end{equation} 
and 
\begin{equation}
\tilde{\beta}_{\theta^*}\left(x_t\right)=\frac{\left(1-\bar{\alpha}_{t-1}\right) \beta_t}{1-\bar{\alpha}_t} \gamma^2.
\label{btheta*}
\end{equation}
Given $\epsilon \sim \mathcal{N}(0, I)$, we define the BGD training optimization as follow:
\begin{equation}
    \begin{aligned}
        % \mathcal{L}_{B G D}\left(\epsilon_{\theta^*}\right) &= \operatorname{MSE}\left(\epsilon-\epsilon_{\theta^*}\left(\sqrt{\bar{\alpha}_t} x_0 \right. \right. \\
        % &\left. \left. + \sqrt{1-\bar{\alpha}_t} \gamma \epsilon+\sqrt{1-\bar{\alpha}_t} \mu, t\right)\right),
        \mathcal{L}_{B G D}\left(\epsilon_{\theta^*}\right) = \operatorname{MSE}\left(\epsilon-\epsilon_{\theta^*}\left(\sqrt{\bar{\alpha}_t} x_0 \right. \right. 
        \left. \left. + \sqrt{1-\bar{\alpha}_t} \gamma \epsilon+\sqrt{1-\bar{\alpha}_t} \mu, t\right)\right),
    \end{aligned}
    \label{lossBGD}
\end{equation}
where $\operatorname{MSE}(\cdot)$ represents the Mean Square Error between. The BGD diffusion and training process is summarized in Algorithm \ref{al1}.
\begin{algorithm}
    \caption{BGD diffusion \& training process}
    \label{al1}
    \begin{algorithmic}
    \REQUIRE
    $x_0 \sim \mathcal{D}$, Trigger $\delta$, Scale factor $\gamma$, Time steps $t \sim \operatorname{Uniform}(\{1, \ldots, T\})$
    \REPEAT
    \STATE $x_t=\sqrt{\bar{\alpha}_t} x_0+\sqrt{1-\bar{\alpha}_t} \gamma \epsilon+\sqrt{1-\bar{\alpha}_t} \mu$
    \STATE Take gradient descent steps on\\
    $\nabla_{\theta^*} \operatorname{MSE}(\epsilon-\epsilon_{\theta^*}(\sqrt{\bar{\alpha}_t} x_0 + \sqrt{1-\bar{\alpha}_t} \gamma \epsilon+\sqrt{1-\bar{\alpha}_t} \mu, t))$
    \UNTIL{Converged}
    \end{algorithmic}
    
\end{algorithm}
%-------------------------------------------------------------------------------------------------------------------
\subsection{Protected image generation}
\label{generation RAE}
The purpose of generating protected images is to obtain slightly noisy images with different model training performance, and then apply reversible adversarial perturbations to them.
%The flowchart for this step is shown in Figure  \hyperref[fig:4]{4}.
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=0.8\linewidth]{image4.png}
%     \caption{The flowchart of the protected image generation \& restoration}
%     \label{fig:4}
% \end{figure*}

Firstly, we define $\mathcal{D}_1^{s n}$ to $\mathcal{D}_m^{s n}$ as the datasets with slight noise for the permission levels from 1 to $m$. The images in these datasets were defined as $x_n^{s n 1}$ to $x_n^{s n m}$. Taking $x_1$ as an example. They arrange the noise levels that differ from clean Images in the following order: 
\begin{equation}
\left\|x_1-x_1^{s n 1}\right\|<\left\|x_1-x_1^{s n 2}\right\|<\cdots<\left\|x_1-x_1^{s n m}\right\|.
\label{clean images order}
\end{equation}
Therefore,  the training performance can be controlled in the user's model by providing datasets with different noise levels.

Given an input $x_0 \sim \mathcal{D}$, we diffuse $x_0$ with $\tilde{q}\left(x_t \mid x_{t-1}\right)$ from $t=1$ to $t=t_m^{s n}$ step by step to generate images $x_n^{s n m}$ in $\mathcal{D}_m^{s n}$, where noise time step $t_m^{s n}$ represents the time step at which the diffusion process stops. As the number of time steps $t_m^{s n}$ increases, the diffusion process introduced by the DDPM on the image will also bring about an increase in the noise. Therefore, theoretically, the size of $t_m^{s n}$ satisfies the following condition:
\begin{equation}
t_1^{s n}<t_2^{s n}<\cdots<t_m^{s n}.    
\label{tsn's orger}
\end{equation}
Secondly, an adverse time step $t_r$ is designated to denoise the $x_n^{s n m}$ adversarially for $t_r$ time steps. To be specific, consider the given $x_n^{s n m}$ as one that has undergone denoising for only $T-t_r$ timesteps. As a result, the DDPM will utilize $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$ to further denoise $x_n^{s n m}$ for $t_r$ time steps.
We modify Equation \eqref{x0theta*} to
\begin{equation}
    x_0^{a d v}=\frac{x_t+\sqrt{1-\bar{\alpha}_t} \gamma \epsilon_{\theta^*}\left(x_t, t\right)+\sqrt{1-\bar{\alpha}_t} \mu}{\sqrt{\bar{\alpha}_t}} , 
    \label{adversarial denoising}
\end{equation}
for the \textbf{AGP} $\tilde{p}_{\theta^*}^{a d v}\left(x_{t-1} \mid x_t\right)$ based on Equation \eqref{ptheta*}:
\begin{equation}
\begin{aligned}
\tilde{p}_{\theta^*}^{a d v}\left(x_{t-1} \mid x_t\right)&=\mathcal{N}\left(x_{t-1} ; \tilde{\mu}_{\theta^*}\left(x_t,x_0^{a d v}\right), \tilde{\beta}_{\theta^*}\left(x_t\right) I\right).\\
\end{aligned}
\label{pthetaadv*}
\end{equation}
If we take the standard generative process performed by DDPM as a way to enhance the semantic representation of the images, the AGP $\tilde{p}_{\theta^*}^{a d v}\left(x_{t-1} \mid x_t\right)$ will gradually steer $x_n^{\text {snm }}$ away from its original semantic representation, giving rise to an adversarial effect.
Finally, $x_n^{p m}$ are generated in protected dataset $\mathcal{D}_m^p$. The values for $t_m^{s n}$ and $t_r$ will be elaborated on in detail in Section \ref{sec:expri}.
It's noteworthy that the perturbation noises introduced on $x_n^{s n m}$ and $x_n^{p m}$ are different.
Because the introduction of perturbation noises involves a crucial parameter $\epsilon$, for generated $x_n^{s n m}$, it is randomly sampled from $z \sim \mathcal{N}(0, I)$, whereas for generated $x_n^{p m}$, it is determined based on prior knowledge parameter $\theta^*$ of DDPM.
Therefore, it ensures that, by introducing varying degrees of slight noise through random sampling, $x_n^{s n m}$ is generated for different training performance permission levels, while simultaneously, based on prior knowledge parameter $\theta^*$ from DDPM, it can self-generate $x_n^{p m}$ with inherent self-recovery capabilities.
% thereby introducing noise influenced by $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$. However, since the $x_n^{s n m}$ essentially serves as the $x_0$ in the training process, the denoising performed by the DDPM on it will not introduce excessive noise. 

The Protected image generation is summarized in Algorithm \hyperref[al2]{2}. 
\begin{algorithm}
    
    \label{al2}
    \caption{Protected image generation}
    \begin{algorithmic}
     \REQUIRE
    $x_0 \sim \mathcal{D}$, Noise time steps $t_m^{s n}$, Trigger $\delta$, Scale factor $\gamma$, Adverse time step $t_r$, Time steps T
    \ENSURE 
    $x_n^{s n m} \sim \mathcal{D}_m^{s n}, x_n^{p m} \sim \mathcal{D}_m^p$
    $\mu=(1-\gamma) \delta$
    \FOR{$m=1, \ldots, m$}{
        \FOR{$n=1, \ldots, n$}{
            \STATE $x_n^{s n m}=\sqrt{\bar{\alpha}_{t_m^{s n}}} x_0+\sqrt{1-\bar{\alpha}_{t_m^{s n}}} \gamma \epsilon+\sqrt{1-\bar{\alpha}_{t_m^{s n}}} \mu$
            \STATE $x_t=x_n^{s n m}$
            \FOR{$t=T, \ldots, 1$}{
            \IF{$t < t_t$}
            \STATE $z \sim \mathcal{N}(0, I)$ if $t>0$, else $z=0$
            \STATE $\quad x_{t-1}=\tilde{\mu}_{\theta^*}\left(x_{t},x_0^{a d v}\right)+\sqrt{\tilde{\beta}_{\theta^*}\left(x_{t}\right) }z$
            \ENDIF
            }
            \ENDFOR
           \STATE $x_n^{p m} = x_0$
        }
        \ENDFOR
    }  
    \ENDFOR
    \end{algorithmic}
    
\end{algorithm}\\
%-------------------------------------------------------------------------------------------------------------------
\subsection{Protected image restoration}
\label{mulu4.5}
The restoration of the protected dataset involves employing the standard generative process $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$ to eliminate the perturbation noise introduced by AGP.
% Authorized users need to provide the trigger $\delta$ to obtain the recovered dataset $\tilde{\mathcal{D}}_m^{s n}$.
% For the standard generative process $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$, as the time steps progress, generated images with progressively richer semantic presentation, thereby bringing images closer to the original ones.
As time steps progress in the standard generative process $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$, images generated showcase a progressively enriched semantic representation, thereby bringing them closer to the original images.
Consequently, the introduced noise for generation gradually diminishes with time steps.
On the contrary, AGP tends to diminish the semantic richness in the generated images as the time steps progress, consequently increasing the introduced noise.
Therefore, relying solely on $t_r$ during the RAE generation is insufficient.
% To further enhance the standard generative process $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$ for RAE generation
An additional parameter, denoted as reverse factor $\eta$, is needed to increase the time steps during the standard generative process $\tilde{p}_{\theta^*}\left(x_{t-1} \mid x_t\right)$ for RAE restoration which is set to \textbf{1.4}.

The Protected image restoration is summarized in Algorithm \hyperref[al3]{3}.

\begin{algorithm}
    
    \label{al3}
    \caption{Protected image restoration}
    \begin{algorithmic}
    \REQUIRE
    $x_n^{p m} \sim \mathcal{D}_m^p$, Time steps $T$, Trigger $\delta$, Scale factor $\gamma$, Adverse time step $t_r$, Reverse factor $\eta$
    \ENSURE$\tilde{x}_n^{s n m} \sim \mathcal{D}_m^{s n}$
    \STATE $\mu=(1-\gamma) \delta$
    \STATE $t_r=\eta t_r$
    \FOR{$t=T, \ldots, 1$}{
        \FOR{$n=1, \ldots, n$}{
        \IF{$t < t_r$}
            \STATE $z \sim \mathcal{N}(0, I)$ if $t>0$, else $z=0$
            \STATE $\quad x_{t-1}=\tilde{\mu}_{\theta^*}\left(x_{t}\right)+\sqrt{\tilde{\beta}_{\theta^*}\left(x_{t}\right) }z$
            \ENDIF
        }
         \STATE $x_n^{p m} = x_0$
        \ENDFOR 
       
    }  
    \ENDFOR
    \end{algorithmic}
    
\end{algorithm}


==> sec/X_biography.tex <==
\newpage

\section{}
\vspace{11pt}
\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{zhaopian/xf.jpg}}]{Fan Xing}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}




\vfill
